Segmentation-free Heart Pathology Detection Using Deep Learning

Cardiovascular (CV) diseases are the leading cause of death in the world, and auscultation is typically an essential part of a cardiovascular examination. The ability to diagnose a patient based on their heart sounds is a rather difficult skill to master. Thus, many approaches for automated heart auscultation have been explored. However, most of the previously proposed methods involve a segmentation step, the performance of which drops significantly for high pulse rates or noisy signals. In this work, we propose a novel segmentation-free heart sound classification method. Specifically, we apply discrete wavelet transform to denoise the signal, followed by feature extraction and feature reduction. Then, Support Vector Machines and Deep Neural Networks are utilised for classification. On the PASCAL heart sound dataset our approach showed superior performance compared to others, achieving 81% and 96% precision on normal and murmur classes, respectively. In addition, for the first time, the data were further explored under a user-independent setting, where the proposed method achieved 92% and 86% precision on normal and murmur, demonstrating the potential of enabling automatic murmur detection for practical use.

==> related-work.tex <==
\section{RELATED WORK}
\cm{given you talk about pascal approaches here i wonder if you should  describe the data before this section: one option is to inlcude the descrption of pascal here...it is after all related work}
\jh{given the page limitation and after checking previous embc papers, i suggest to shorten content in this section and merge it into the introduction, which can follow like this: introduce the research topic, murmur detection, conventional approaches, in particular issue of existing segmentation-based approach, the proposed segment-free approach, contribution of the work, findings including the better performance than SOTA on Pascal and the performance decrease in user-independent settings. Moreover, I would say it is unnecessary to discuss SVM and NN cons and pros, as this is not focus of this work?}
\subsection{Heart sound preprocessing}

Deep learning is rapidly gaining popularity due to its ability to learn from raw data~\cite{Lecun2015}. However, in the case of some medical data, such as heart sounds, sample scarcity forces researchers to resort to signal processing techniques: denoising, segmentation, and feature extraction.\cm{perhaps a bit narrow: i think it woudl be best if we were not just meaning that as soon as data is large this approach is useless:)}

Most common segmentation approaches include envelope-based methods and probabilistic methods. Envelope-based heart sound segmentation offers several approaches:  normalised Shannon average energy~\cite{Gomes2012, Balili2015, Chakir2018} and Hilbert transform and its variations~\cite{Huang1998, Cherif2013, Sharma2015}. However, these methods are based on the premise that systole is shorter than diastole, which is only true for a narrow band of heart rates~\cite{Deng2012}. Probabilistic methods, another popular approach to segmentation, are based on the idea that it is possible to discriminate the fundamental heart sounds based on some discriminative features, such as temporal correlation, waveform function, etc. Especially popular are Hidden Markov Model-based segmentation methods~\cite{Wang2007, Springer2015}, however they are not as effective for signals with high levels of noise.\cm{any possible citation?}

Ultimately, it is important to be aware of the segmentation's limitations: its reliance on the signal being clean~\cite{Banerjee2020} within a narrow band of heart rates drastically limits its application, the error introduced by incorrect segmentation will propagate into heart sound pathology classification, and introduce considerable computational complexity into the algorithms~\cite{Langley2017}. Considering these disadvantages of segmentation, segmentation-free methods show more promise.

\subsection{Heart sound classification}

Numerous approaches have been studied for heart sound classification, with the majority of methods based on support vector machines (SVMs) and neural networks (NNs)\cm{again be consistent with abstact, also you have already defined these acronyms..perhpas save space?}.
%\jh{better to cite?}.

SVMs are a very popular approach for heart sound classification, with a majority of research attempts using various feature inputs. The main advantage of SVM over a neural network is its lesser sensitivity to the training set size --- SVMs are known to deal better with small sample sizes~\cite{Dwivedi2019}. The main disadvantage of SVM is its complexity for multi-class problems since a different model is required for each class. Some of the approaches using SVMs included utilising deep features as an input, which yielded a sensitivity of 84.8\%~\cite{Tschannen2016}, and using sparse coding for feature extraction, achieving 86.5\% accuracy~\cite{Whitaker2016}, both on PhysioNet heart sound dataset. 

Neural networks are also very popular as a classification approach for heart sound signals, exploited by numerous research groups~\cite{Degroff2001, Olmez2003, Nilanon2016}. %They are an especially attractive algorithm choice due to its ability to detect trends based on sample data, self-organisation properties, and real-time operation. 
While NNs deal exceptionally well with multi-class problems, unlike SVMs they require large datasets. However, there is a clear lack of studies comparing the inferential capabilities of SVMs and NNs on the same heart sounds data.%\cm{you mean in general or heart data? the former is probably not true} \eb{very well spotted, indeed mean only for heart sound data}

The PASCAL heart sound challenge involved two sub-challenges, heart sound segmentation and classification, but in this work the latter is of particular interest. The two winners of the challenge proposed employing segmentation-based features, with the first group utilising J48 and multi-layer perceptron (MLP) algorithms~\cite{Gomes2012}, while the second group proposed an algorithmic approach (no machine learning)~\cite{Deng2012}. Few years later, Balili et al.~\cite{Balili2015} explored using discrete and continuous wavelet transform coefficients as an input to a random forest classifier. This approach was followed by a study from Chakir et al.~\cite{Chakir2018}, where segmentation-based features and a discriminant analysis classifier were used. 

\subsection{Segmentation-free classification}
\eb{Still unsure if I should include this section, given that there are no segmentation-free approaches on PASCAL to the best of my knowledge, and others are not as interesting since they don't do extrasys. Will still look into this, and see if I find something worth including here.}
\cm{I think we need to say something as people will ask if you are the first segmentation free approach to this problem}

\cm{the related work section should end with a statement of contribuiton/novelty
}

\jh{how about the one with 2.03 total precision?}
